Multi-Step Model Predictive Safety Filters: Reducing Chattering by Increasing the Prediction Horizon

Learning-based controllers have demonstrated superior performance compared to classical controllers in various tasks. However, providing safety guarantees is not trivial. Safety, the satisfaction of state and input constraints, can be guaranteed by augmenting the learned control policy with a safety filter. Model predictive safety filters (MPSFs) are a common safety filtering approach based on model predictive control (MPC). MPSFs seek to guarantee safety while minimizing the difference between the proposed and applied inputs in the immediate next time step. This limited foresight can lead to jerky motions and undesired oscillations close to constraint boundaries, known as chattering. In this paper, we reduce chattering by considering input corrections over a longer horizon. Under the assumption of bounded model uncertainties, we prove recursive feasibility using techniques from robust MPC. We verified the proposed approach in both extensive simulation and quadrotor experiments. In experiments with a Crazyflie 2.0 drone, we show that, in addition to preserving the desired safety guarantees, the proposed MPSF reduces chattering by more than a factor of 4 compared to previous MPSF formulations.

==> figs/chattering_example/chatter_1s.tex <==
% This file was created with tikzplotlib v0.10.1.
\begin{tikzpicture}

\definecolor{cornflowerblue}{RGB}{100,149,237}
\definecolor{darkgray176}{RGB}{176,176,176}
\definecolor{plum}{RGB}{221,160,221}

\begin{axis}[
height=1.9in,
tick align=outside,
tick pos=left,
width=1.9in,
x grid style={darkgray176},
xlabel={Angle $\theta$ [\unit{\radian}]},
xmin=0.15, xmax=0.163,
xtick style={color=black},
y grid style={darkgray176},
ylabel={Angular Velocity $\dot{\theta}$ [\unit{\radian\per\second}]},
ymin=-0.2, ymax=0.2,
ytick style={color=black}
]
\addplot [semithick, plum, dash pattern=on 5.55pt off 2.4pt]
table {%
0 0
-0.0176028713137575 -0.520675770777488
-0.0559794071461549 -0.634991527003369
-0.095727253026992 -0.565836624333742
-0.128506838704594 -0.426227726576724
-0.151492827188353 -0.270642461375219
-0.164457976371896 -0.123626922210557
-0.168308518487966 0.00482667867262113
-0.164380367645839 0.111580209403021
-0.154108908340437 0.196697080926468
-0.138874568685888 0.261744266443066
-0.119930866691576 0.308977376911933
-0.0983733759005351 0.340908927037812
-0.0751314236302291 0.360048592604709
-0.0509738337653588 0.368736727950398
-0.0265234683964353 0.369044286056251
-0.00227659945785077 0.362726654035561
0.0213760653690587 0.351219627113445
0.0441290554967272 0.335664366827206
0.0657440071882065 0.316948677406194
0.0860344699986971 0.295754368549398
0.10485381904669 0.272603698420707
0.122086077772777 0.247900880681263
0.1376392649592 0.221966889300145
0.151440810976528 0.195067233910477
0.163434592799239 0.167433159712051
0.17357917878319 0.139277062355088
0.181846929313987 0.110802987577497
0.188223655690179 0.0822130425717088
0.192708591714468 0.0537104651137257
0.195314479393714 0.0255000220036284
0.196067612901265 -0.00221364237226706
0.195007725094589 -0.0292291140009321
0.192187639588781 -0.0553521955673614
0.187672648952963 -0.0804002118495107
0.18153961526276 -0.104206113269523
0.173875821343551 -0.126621926079115
0.16477762740239 -0.147521201935831
0.154349006240003 -0.166800253569012
0.142700039345115 -0.184378113308546
0.129945455456478 -0.200195298639661
0.116203283458725 -0.214211594044043
0.101593674750429 -0.226403145457042
0.0862379292787255 -0.236759204325444
0.0702577373343762 -0.245278852785559
0.053774628729969 -0.251967997889884
0.036909604234417 -0.256836854052816
0.01978291229324 -0.259898053443475
0.00251392740477102 -0.261165446823501
-0.0147789154072671 -0.260653591576532
-0.0319781737071469 -0.258377874296152
-0.0489674774581057 -0.254355183175664
-0.065631668452332 -0.248605028509565
-0.0818570253535457 -0.2411510041374
-0.097531593298074 -0.232022484392875
-0.112545630181615 -0.221256456170188
-0.126792175288868 -0.20889939105155
-0.140167739757128 -0.195009066108984
-0.152573112366436 -0.179656243177991
-0.163914268162102 -0.162926115334754
-0.174103361330554 -0.144919427164516
-0.183059777559684 -0.125753174145819
-0.190711214961291 -0.10556078863718
-0.196994756834169 -0.084491728377884
-0.201857894602812 -0.062710400823183
-0.205259455836949 -0.0403943850794575
-0.207170391091611 -0.0177319534285703
-0.207574375141467 0.00508105477632113
-0.206468183593502 0.0278448963184122
-0.203861815105362 0.0503599553151156
-0.199778342302096 0.0724309219469905
-0.194253490200193 0.0938708630683968
-0.187334958184425 0.114504918047038
-0.179081518571923 0.134173371578381
-0.169561939573697 0.1527339037722
-0.158853791185353 0.17006289197053
};
\addplot [semithick, cornflowerblue, mark=*, mark size=1, mark options={solid}]
table {%
0 0
-0.0176028713113121 -0.520675770705161
-0.0559794071371873 -0.634991526879949
-0.0957272530087523 -0.565836624178026
-0.128506838675154 -0.426227726394963
-0.151492827144788 -0.270642461131891
-0.159575256670767 0.0207965260035107
-0.157722822799116 0.0348226945994673
-0.153553314317856 0.0898990326104446
-0.145373860226516 0.155623867971738
-0.132973831863521 0.21734472396487
-0.116832908865428 0.268713055718
-0.0977052480564859 0.307710092947652
-0.0764046817137983 0.334514062351692
-0.0536984877742562 0.350334708501168
-0.0302607701577139 0.356768515409394
-0.00665864430147606 0.355447650713169
0.0166441532240542 0.347862164252453
0.0392753654597068 0.335286020236909
0.0609394464434845 0.318763625743815
0.0814029885048509 0.299128792870749
0.100481893696162 0.277038241417736
0.118030890921315 0.253008863411299
0.133935449451891 0.227452837709445
0.148105852939326 0.200707814560617
0.159732933557809 0.151174282001448
0.159571563481693 -0.14998459549134
0.156708416548194 0.0593933550313927
0.159750750834618 0.0329492646884951
0.159726224629411 -0.0323751450964968
0.159812249307756 0.0336428691057053
0.159724119896858 -0.0349230227019246
0.159815625715052 0.0362523835907229
0.15972063548494 -0.0376325807871941
0.159819240502872 0.0390650618935147
0.159716880143235 -0.0405523579267838
0.159606552243596 0.0356896249684995
0.159725439008354 -0.030764694773127
0.158067648503304 -0.0194883237540875
0.155813295486382 -0.0479698964832888
0.151166319405335 -0.0913934220655262
0.143560782501862 -0.137204660701178
0.13304144089337 -0.179394773649016
0.119934443544268 -0.215411171051716
0.104674370107318 -0.244499313105527
0.0877152939880401 -0.266808923172913
0.0694872601745913 -0.282908465726722
0.0503774556416896 -0.293520808092331
0.0307247473369584 -0.29938165179315
0.0108212397644637 -0.301167924579786
-0.00908278954217572 -0.299466731354188
-0.0287726857016917 -0.294767730799703
-0.0480631452670969 -0.287468547872469
-0.0667925253824974 -0.277886792775648
-0.0848180379533911 -0.266274730405927
-0.10201192534157 -0.252834248696668
-0.118258593398235 -0.237730818778329
-0.133452613346816 -0.221105803495366
-0.147497474852933 -0.203086871116797
-0.159741653099923 -0.167139145720823
-0.159550439844946 0.166202581135337
-0.156757508465466 -0.0770517962165629
-0.159726661870209 -0.0138261880928431
-0.159751742674195 0.012538879356504
-0.159785782216283 -0.0130512519305656
-0.159751608053127 0.0135474238319243
-0.159787105416204 -0.0140631409519736
-0.159750256978326 0.0145985133738509
-0.15978850795845 -0.0151542275415756
-0.159748800611964 0.0157311388572217
-0.159790019291934 -0.0163299666772431
-0.159747231232299 0.0169516397483339
-0.159791647863304 -0.0175969260122522
-0.159745540068368 0.0182668340472384
-0.159793402764341 -0.0189621829712599
-0.159743717665297 0.0196840687444687
};
\addplot [semithick, red, mark=*, mark size=1, mark options={solid}, only marks]
table {%
-0.151492827144788 -0.270642461131891
0.148105852939326 0.200707814560617
0.159732933557809 0.151174282001448
0.156708416548194 0.0593933550313927
0.159750750834618 0.0329492646884951
0.159726224629411 -0.0323751450964968
0.159812249307756 0.0336428691057053
0.159724119896858 -0.0349230227019246
0.159815625715052 0.0362523835907229
0.15972063548494 -0.0376325807871941
0.159819240502872 0.0390650618935147
0.159606552243596 0.0356896249684995
-0.159741653099923 -0.167139145720823
-0.156757508465466 -0.0770517962165629
-0.159726661870209 -0.0138261880928431
-0.159751742674195 0.012538879356504
-0.159785782216283 -0.0130512519305656
-0.159751608053127 0.0135474238319243
-0.159787105416204 -0.0140631409519736
-0.159750256978326 0.0145985133738509
-0.15978850795845 -0.0151542275415756
-0.159748800611964 0.0157311388572217
-0.159790019291934 -0.0163299666772431
-0.159747231232299 0.0169516397483339
-0.159791647863304 -0.0175969260122522
-0.159745540068368 0.0182668340472384
-0.159793402764341 -0.0189621829712599
};
\addplot [line width=2pt, black]
table {%
-0.16 -0.2
-0.16 0.2
};
\addplot [line width=2pt, black]
table {%
0.16 -0.2
0.16 0.2
};
\end{axis}

\end{tikzpicture}


==> figs/chattering_example/chatter_pre_2.tex <==
% This file was created with tikzplotlib v0.10.1.
\begin{tikzpicture}

\definecolor{darkgray176}{RGB}{176,176,176}
\definecolor{limegreen}{RGB}{50,205,50}
\definecolor{plum}{RGB}{221,160,221}

\begin{axis}[
height=1.9in,
tick align=outside,
tick pos=left,
width=1.9in,
x grid style={darkgray176},
xlabel={Angle $\theta$ [\unit{\radian}]},
xmin=0.15, xmax=0.163,
xtick style={color=black},
y grid style={darkgray176},
ymin=-0.2, ymax=0.2,
ytick=\empty
]
\addplot [semithick, plum, dash pattern=on 5.55pt off 2.4pt]
table {%
0 0
-0.0176028713137575 -0.520675770777488
-0.0559794071461549 -0.634991527003369
-0.095727253026992 -0.565836624333742
-0.128506838704594 -0.426227726576724
-0.151492827188353 -0.270642461375219
-0.164457976371896 -0.123626922210557
-0.168308518487966 0.00482667867262113
-0.164380367645839 0.111580209403021
-0.154108908340437 0.196697080926468
-0.138874568685888 0.261744266443066
-0.119930866691576 0.308977376911933
-0.0983733759005351 0.340908927037812
-0.0751314236302291 0.360048592604709
-0.0509738337653588 0.368736727950398
-0.0265234683964353 0.369044286056251
-0.00227659945785077 0.362726654035561
0.0213760653690587 0.351219627113445
0.0441290554967272 0.335664366827206
0.0657440071882065 0.316948677406194
0.0860344699986971 0.295754368549398
0.10485381904669 0.272603698420707
0.122086077772777 0.247900880681263
0.1376392649592 0.221966889300145
0.151440810976528 0.195067233910477
0.163434592799239 0.167433159712051
0.17357917878319 0.139277062355088
0.181846929313987 0.110802987577497
0.188223655690179 0.0822130425717088
0.192708591714468 0.0537104651137257
0.195314479393714 0.0255000220036284
0.196067612901265 -0.00221364237226706
0.195007725094589 -0.0292291140009321
0.192187639588781 -0.0553521955673614
0.187672648952963 -0.0804002118495107
0.18153961526276 -0.104206113269523
0.173875821343551 -0.126621926079115
0.16477762740239 -0.147521201935831
0.154349006240003 -0.166800253569012
0.142700039345115 -0.184378113308546
0.129945455456478 -0.200195298639661
0.116203283458725 -0.214211594044043
0.101593674750429 -0.226403145457042
0.0862379292787255 -0.236759204325444
0.0702577373343762 -0.245278852785559
0.053774628729969 -0.251967997889884
0.036909604234417 -0.256836854052816
0.01978291229324 -0.259898053443475
0.00251392740477102 -0.261165446823501
-0.0147789154072671 -0.260653591576532
-0.0319781737071469 -0.258377874296152
-0.0489674774581057 -0.254355183175664
-0.065631668452332 -0.248605028509565
-0.0818570253535457 -0.2411510041374
-0.097531593298074 -0.232022484392875
-0.112545630181615 -0.221256456170188
-0.126792175288868 -0.20889939105155
-0.140167739757128 -0.195009066108984
-0.152573112366436 -0.179656243177991
-0.163914268162102 -0.162926115334754
-0.174103361330554 -0.144919427164516
-0.183059777559684 -0.125753174145819
-0.190711214961291 -0.10556078863718
-0.196994756834169 -0.084491728377884
-0.201857894602812 -0.062710400823183
-0.205259455836949 -0.0403943850794575
-0.207170391091611 -0.0177319534285703
-0.207574375141467 0.00508105477632113
-0.206468183593502 0.0278448963184122
-0.203861815105362 0.0503599553151156
-0.199778342302096 0.0724309219469905
-0.194253490200193 0.0938708630683968
-0.187334958184425 0.114504918047038
-0.179081518571923 0.134173371578381
-0.169561939573697 0.1527339037722
-0.158853791185353 0.17006289197053
};
\addplot [semithick, limegreen, mark=*, mark size=1, mark options={solid}]
table {%
0 0
-0.017602871307096 -0.520675770580458
-0.0559794071226658 -0.63499152669494
-0.0957272529804744 -0.565836623948824
-0.128506838626375 -0.426227726008684
-0.149979282759855 -0.225891322266875
-0.159537186312807 -0.065806982083676
-0.15968732479015 0.0587690312785015
-0.154329204879072 0.102058550299655
-0.14555684102218 0.161482709385387
-0.132880524864092 0.219889168495878
-0.116628367499042 0.26955872412076
-0.0974727356818441 0.307724736834395
-0.0761837268820781 0.334157881572115
-0.053505610889159 0.349846191297739
-0.0301007386768873 0.356266173394769
-0.00653053851168275 0.354985828127934
0.0167437207916475 0.347461629474987
0.0393505879089919 0.334950641585772
0.0609945056762429 0.318489351654131
0.0814416901289495 0.29890838447761
0.100507536983245 0.276863676810352
0.118046255575411 0.252872482025628
0.133942835689256 0.227347817300342
0.147818861408044 0.192103899700366
0.156644787247394 0.0765905499266157
0.159729458522511 0.0176862293881743
0.159746632421405 -0.0164805622280631
0.15946393356857 0.00746806418586703
0.159765178523237 0.0017378884258738
0.159766825576517 -0.00162061907063627
0.159771191777757 0.00168585761606903
0.159766776805649 -0.00174996616344379
0.15977136210511 0.00181658424393902
0.159766602294193 -0.00188573758999938
0.159771543297584 0.00195752282635717
0.159766414177135 -0.00203204207945054
0.159771738544039 0.00210939723511035
0.159519054453916 -0.00950111743126658
0.157561943493378 -0.0487707834571095
0.152710554399335 -0.0966722281263641
0.144711634984261 -0.143772090831505
0.133765149690579 -0.185722539765407
0.120269003356384 -0.220844602338531
0.104685943107546 -0.248834212752659
0.0874760460973655 -0.27006406476751
0.0690647110470688 -0.285203443032946
0.0498299887403037 -0.295011119100957
0.0301003586060343 -0.300225259577496
0.0101579173764699 -0.301509146250254
-0.00975594353794001 -0.2994297853767
-0.0294340783417736 -0.294455394559974
-0.0486973153534192 -0.286963448237752
-0.0673888910427564 -0.277253866103837
-0.0853698192470062 -0.265564040375479
-0.102515250996301 -0.252083727398529
-0.118711779594524 -0.236968723065165
-0.133855593048307 -0.220352808273525
-0.147524309507194 -0.192687170695129
-0.156412843425666 -0.077882238226243
-0.159573168123451 -0.0186836006782585
-0.159748365243013 0.0127638380193098
-0.159546674014062 -0.00629417424296971
-0.15976510710152 -0.00041574750456843
-0.159768558427116 0.000297253316012083
-0.159769425052166 -0.000311165203962172
-0.159768611434075 0.000322960355727667
-0.159769457688737 -0.000335255709779839
-0.159768579252411 0.000348018112120638
-0.159769491130333 -0.000361266377692092
-0.159768544539775 0.000375018979675951
-0.159769527165189 -0.000389295099317334
-0.159768507133484 0.000404114700505432
-0.159769565999367 -0.000419498539831468
-0.159768466823967 0.000435468055686212
-0.159769607833365 -0.000452045190314419
};
\addplot [semithick, red, mark=*, mark size=1, mark options={solid}, only marks]
table {%
-0.128506838626375 -0.426227726008684
-0.149979282759855 -0.225891322266875
-0.159537186312807 -0.065806982083676
0.147818861408044 0.192103899700366
0.156644787247394 0.0765905499266157
0.159729458522511 0.0176862293881743
0.159746632421405 -0.0164805622280631
0.15946393356857 0.00746806418586703
0.159765178523237 0.0017378884258738
0.159766825576517 -0.00162061907063627
0.159771191777757 0.00168585761606903
0.159766776805649 -0.00174996616344379
0.15977136210511 0.00181658424393902
0.159766602294193 -0.00188573758999938
0.159771543297584 0.00195752282635717
0.159766414177135 -0.00203204207945054
-0.147524309507194 -0.192687170695129
-0.156412843425666 -0.077882238226243
-0.159573168123451 -0.0186836006782585
-0.159748365243013 0.0127638380193098
-0.159546674014062 -0.00629417424296971
-0.15976510710152 -0.00041574750456843
-0.159768558427116 0.000297253316012083
-0.159769425052166 -0.000311165203962172
-0.159768611434075 0.000322960355727667
-0.159769457688737 -0.000335255709779839
-0.159768579252411 0.000348018112120638
-0.159769491130333 -0.000361266377692092
-0.159768544539775 0.000375018979675951
-0.159769527165189 -0.000389295099317334
-0.159768507133484 0.000404114700505432
-0.159769565999367 -0.000419498539831468
-0.159768466823967 0.000435468055686212
};
\addplot [line width=2pt, black]
table {%
-0.16 -0.2
-0.16 0.2
};
\addplot [line width=2pt, black]
table {%
0.16 -0.2
0.16 0.2
};
\end{axis}

\end{tikzpicture}


==> figs/real_experiments/magnitude_of_corrections.tex <==
% This file was created with tikzplotlib v0.10.1.
\begin{tikzpicture}

\definecolor{cornflowerblue}{RGB}{100,149,237}
\definecolor{darkgray176}{RGB}{176,176,176}
\definecolor{darkgreen}{RGB}{0,100,0}
\definecolor{forestgreen}{RGB}{34,139,34}
\definecolor{limegreen}{RGB}{50,205,50}
\definecolor{pink}{RGB}{255,192,203}

\begin{axis}[
height=2.2in,
tick align=outside,
tick pos=left,
width=3.5in,
x grid style={darkgray176},
xmin=0.5, xmax=5.5,
xtick style={color=black},
tick label style={font=\small},
xtick={1,2,3,4,5},
xticklabels={
  {\(\displaystyle J_{\text{MPSF}, 1}\)},
  {\(\displaystyle +J_{\text{reg}, 10}\)},
  {\(\displaystyle \bm{J_{\text{MPSF}, 2}}\)},
  {\(\displaystyle \bm{J_{\text{MPSF}, 5}}\)},
  {\(\displaystyle \bm{J_{\text{MPSF}, 10}}\)}
},
y grid style={darkgray176},
ylabel={Magnitude Of Corrections},
ymajorgrids,
ymin=0, ymax=3.29834899891414,
ytick style={color=black}
]
\path [draw=black, fill=cornflowerblue]
(axis cs:0.625,2.89185720947142)
--(axis cs:1.375,2.89185720947142)
--(axis cs:1.375,3.0347769057616)
--(axis cs:0.625,3.0347769057616)
--(axis cs:0.625,2.89185720947142)
--cycle;
\addplot [black]
table {%
1 2.89185720947142
1 2.69179682643695
};
\addplot [black]
table {%
1 3.0347769057616
1 3.23598237071036
};
\addplot [black]
table {%
0.8125 2.69179682643695
1.1875 2.69179682643695
};
\addplot [black]
table {%
0.8125 3.23598237071036
1.1875 3.23598237071036
};
\path [draw=black, fill=pink]
(axis cs:1.625,2.65555157938109)
--(axis cs:2.375,2.65555157938109)
--(axis cs:2.375,2.6977450420146)
--(axis cs:1.625,2.6977450420146)
--(axis cs:1.625,2.65555157938109)
--cycle;
\addplot [black]
table {%
2 2.65555157938109
2 2.64740705588423
};
\addplot [black]
table {%
2 2.6977450420146
2 2.69877516435494
};
\addplot [black]
table {%
1.8125 2.64740705588423
2.1875 2.64740705588423
};
\addplot [black]
table {%
1.8125 2.69877516435494
2.1875 2.69877516435494
};
\path [draw=black, fill=limegreen]
(axis cs:2.625,2.85599803626676)
--(axis cs:3.375,2.85599803626676)
--(axis cs:3.375,2.98303823802469)
--(axis cs:2.625,2.98303823802469)
--(axis cs:2.625,2.85599803626676)
--cycle;
\addplot [black]
table {%
3 2.85599803626676
3 2.85599803626676
};
\addplot [black]
table {%
3 2.98303823802469
3 3.07785488725556
};
\addplot [black]
table {%
2.8125 2.85599803626676
3.1875 2.85599803626676
};
\addplot [black]
table {%
2.8125 3.07785488725556
3.1875 3.07785488725556
};
\addplot [black, mark=o, mark size=1.5, mark options={solid,fill opacity=0}, only marks]
table {%
3 2.64851447750205
};
\path [draw=black, fill=forestgreen]
(axis cs:3.625,2.47718661081538)
--(axis cs:4.375,2.47718661081538)
--(axis cs:4.375,2.56605296976457)
--(axis cs:3.625,2.56605296976457)
--(axis cs:3.625,2.47718661081538)
--cycle;
\addplot [black]
table {%
4 2.47718661081538
4 2.36193025275146
};
\addplot [black]
table {%
4 2.56605296976457
4 2.62943404233299
};
\addplot [black]
table {%
3.8125 2.36193025275146
4.1875 2.36193025275146
};
\addplot [black]
table {%
3.8125 2.62943404233299
4.1875 2.62943404233299
};
\path [draw=black, fill=darkgreen]
(axis cs:4.625,1.99815492400848)
--(axis cs:5.375,1.99815492400848)
--(axis cs:5.375,2.02282401713005)
--(axis cs:4.625,2.02282401713005)
--(axis cs:4.625,1.99815492400848)
--cycle;
\addplot [black]
table {%
5 1.99815492400848
5 1.98864980663465
};
\addplot [black]
table {%
5 2.02282401713005
5 2.02282401713005
};
\addplot [black]
table {%
4.8125 1.98864980663465
5.1875 1.98864980663465
};
\addplot [black]
table {%
4.8125 2.02282401713005
5.1875 2.02282401713005
};
\addplot [black, mark=o, mark size=1.5, mark options={solid,fill opacity=0}, only marks]
table {%
5 2.12979815327947
};
\addplot [line width=1pt, black, dash pattern=on 9.25pt off 4pt]
table {%
0.625 2.9659856850882
1.375 2.9659856850882
};
\addplot [line width=1pt, black, dash pattern=on 9.25pt off 4pt]
table {%
1.625 2.6664561839795
2.375 2.6664561839795
};
\addplot [line width=1pt, black, dash pattern=on 9.25pt off 4pt]
table {%
2.625 2.88426755350186
3.375 2.88426755350186
};
\addplot [line width=1pt, black, dash pattern=on 9.25pt off 4pt]
table {%
3.625 2.50291160663171
4.375 2.50291160663171
};
\addplot [line width=1pt, black, dash pattern=on 9.25pt off 4pt]
table {%
4.625 2.01582188697038
5.375 2.01582188697038
};
\end{axis}

\end{tikzpicture}


==> figs/real_experiments/max_correction.tex <==
% This file was created with tikzplotlib v0.10.1.
\begin{tikzpicture}

\definecolor{cornflowerblue}{RGB}{100,149,237}
\definecolor{darkgray176}{RGB}{176,176,176}
\definecolor{darkgreen}{RGB}{0,100,0}
\definecolor{forestgreen}{RGB}{34,139,34}
\definecolor{limegreen}{RGB}{50,205,50}
\definecolor{pink}{RGB}{255,192,203}

\begin{axis}[
height=2.2in,
tick align=outside,
tick pos=left,
width=3.5in,
x grid style={darkgray176},
xmin=0.5, xmax=5.5,
xtick style={color=black},
tick label style={font=\small},
xtick={1,2,3,4,5},
xticklabels={
  {\(\displaystyle J_{\text{MPSF}, 1}\)},
  {\(\displaystyle +J_{\text{reg}, 10}\)},
  {\(\displaystyle \bm{J_{\text{MPSF}, 2}}\)},
  {\(\displaystyle \bm{J_{\text{MPSF}, 5}}\)},
  {\(\displaystyle \bm{J_{\text{MPSF}, 10}}\)}
},
y grid style={darkgray176},
ylabel={Max Correction},
ymajorgrids,
ymin=0, ymax=0.505593469859257,
ytick style={color=black}
]
\path [draw=black, fill=cornflowerblue]
(axis cs:0.625,0.445734208055108)
--(axis cs:1.375,0.445734208055108)
--(axis cs:1.375,0.450885935830959)
--(axis cs:0.625,0.450885935830959)
--(axis cs:0.625,0.445734208055108)
--cycle;
\addplot [black]
table {%
1 0.445734208055108
1 0.445334077995374
};
\addplot [black]
table {%
1 0.450885935830959
1 0.450885935830959
};
\addplot [black]
table {%
0.8125 0.445334077995374
1.1875 0.445334077995374
};
\addplot [black]
table {%
0.8125 0.450885935830959
1.1875 0.450885935830959
};
\addplot [black, mark=o, mark size=1.5, mark options={solid,fill opacity=0}, only marks]
table {%
1 0.494957441076353
};
\path [draw=black, fill=pink]
(axis cs:1.625,0.440137448681836)
--(axis cs:2.375,0.440137448681836)
--(axis cs:2.375,0.441955778001346)
--(axis cs:1.625,0.441955778001346)
--(axis cs:1.625,0.440137448681836)
--cycle;
\addplot [black]
table {%
2 0.440137448681836
2 0.43994556159441
};
\addplot [black]
table {%
2 0.441955778001346
2 0.443355982410079
};
\addplot [black]
table {%
1.8125 0.43994556159441
2.1875 0.43994556159441
};
\addplot [black]
table {%
1.8125 0.443355982410079
2.1875 0.443355982410079
};
\path [draw=black, fill=limegreen]
(axis cs:2.625,0.444363957844869)
--(axis cs:3.375,0.444363957844869)
--(axis cs:3.375,0.445726539504772)
--(axis cs:2.625,0.445726539504772)
--(axis cs:2.625,0.444363957844869)
--cycle;
\addplot [black]
table {%
3 0.444363957844869
3 0.443023048112823
};
\addplot [black]
table {%
3 0.445726539504772
3 0.445726539504772
};
\addplot [black]
table {%
2.8125 0.443023048112823
3.1875 0.443023048112823
};
\addplot [black]
table {%
2.8125 0.445726539504772
3.1875 0.445726539504772
};
\addplot [black, mark=o, mark size=1.5, mark options={solid,fill opacity=0}, only marks]
table {%
3 0.450119367053481
};
\path [draw=black, fill=forestgreen]
(axis cs:3.625,0.398493907956146)
--(axis cs:4.375,0.398493907956146)
--(axis cs:4.375,0.442051646254381)
--(axis cs:3.625,0.442051646254381)
--(axis cs:3.625,0.398493907956146)
--cycle;
\addplot [black]
table {%
4 0.398493907956146
4 0.384243004736605
};
\addplot [black]
table {%
4 0.442051646254381
4 0.442324173519583
};
\addplot [black]
table {%
3.8125 0.384243004736605
4.1875 0.384243004736605
};
\addplot [black]
table {%
3.8125 0.442324173519583
4.1875 0.442324173519583
};
\path [draw=black, fill=darkgreen]
(axis cs:4.625,0.288068681407855)
--(axis cs:5.375,0.288068681407855)
--(axis cs:5.375,0.313746755135147)
--(axis cs:4.625,0.313746755135147)
--(axis cs:4.625,0.288068681407855)
--cycle;
\addplot [black]
table {%
5 0.288068681407855
5 0.282236865418274
};
\addplot [black]
table {%
5 0.313746755135147
5 0.345043163195458
};
\addplot [black]
table {%
4.8125 0.282236865418274
5.1875 0.282236865418274
};
\addplot [black]
table {%
4.8125 0.345043163195458
5.1875 0.345043163195458
};
\addplot [line width=1pt, black, dash pattern=on 9.25pt off 4pt]
table {%
0.625 0.446833162327541
1.375 0.446833162327541
};
\addplot [line width=1pt, black, dash pattern=on 9.25pt off 4pt]
table {%
1.625 0.440585352084996
2.375 0.440585352084996
};
\addplot [line width=1pt, black, dash pattern=on 9.25pt off 4pt]
table {%
2.625 0.445682282193976
3.375 0.445682282193976
};
\addplot [line width=1pt, black, dash pattern=on 9.25pt off 4pt]
table {%
3.625 0.439265624403065
4.375 0.439265624403065
};
\addplot [line width=1pt, black, dash pattern=on 9.25pt off 4pt]
table {%
4.625 0.291528661479677
5.375 0.291528661479677
};
\end{axis}

\end{tikzpicture}


==> figs/real_experiments/rate_of_change_of_inputs.tex <==
% This file was created with tikzplotlib v0.10.1.
\begin{tikzpicture}

\definecolor{cornflowerblue}{RGB}{100,149,237}
\definecolor{darkgray176}{RGB}{176,176,176}
\definecolor{darkgreen}{RGB}{0,100,0}
\definecolor{forestgreen}{RGB}{34,139,34}
\definecolor{limegreen}{RGB}{50,205,50}
\definecolor{pink}{RGB}{255,192,203}
\definecolor{plum}{RGB}{221,160,221}

\begin{axis}[
height=2.2in,
tick align=outside,
tick pos=left,
width=3.5in,
x grid style={darkgray176},
xmin=0.5, xmax=6.5,
xtick style={color=black},
tick label style={font=\small},
xtick={1,2,3,4,5,6},
xticklabels={
  Uncert,
  {\(\displaystyle J_{\text{MPSF}, 1}\)},
  {\(\displaystyle +J_{\text{reg}, 10}\)},
  {\(\displaystyle \bm{J_{\text{MPSF}, 2}}\)},
  {\(\displaystyle \bm{J_{\text{MPSF}, 5}}\)},
  {\(\displaystyle \bm{J_{\text{MPSF}, 10}}\)}
},
y grid style={darkgray176},
ylabel={Rate Of Change Of Inputs},
ymajorgrids,
ymin=0, ymax=40.4932027033441,
ytick style={color=black}
]
\path [draw=black, fill=plum]
(axis cs:0.625,2.56795103632871)
--(axis cs:1.375,2.56795103632871)
--(axis cs:1.375,2.60656192783189)
--(axis cs:0.625,2.60656192783189)
--(axis cs:0.625,2.56795103632871)
--cycle;
\addplot [black]
table {%
1 2.56795103632871
1 2.55375999958099
};
\addplot [black]
table {%
1 2.60656192783189
1 2.61545322089037
};
\addplot [black]
table {%
0.8125 2.55375999958099
1.1875 2.55375999958099
};
\addplot [black]
table {%
0.8125 2.61545322089037
1.1875 2.61545322089037
};
\path [draw=black, fill=cornflowerblue]
(axis cs:1.625,27.0726731286697)
--(axis cs:2.375,27.0726731286697)
--(axis cs:2.375,31.3736864181965)
--(axis cs:1.625,31.3736864181965)
--(axis cs:1.625,27.0726731286697)
--cycle;
\addplot [black]
table {%
2 27.0726731286697
2 26.7910504058682
};
\addplot [black]
table {%
2 31.3736864181965
2 31.3736864181965
};
\addplot [black]
table {%
1.8125 26.7910504058682
2.1875 26.7910504058682
};
\addplot [black]
table {%
1.8125 31.3736864181965
2.1875 31.3736864181965
};
\addplot [black, mark=o, mark size=1.5, mark options={solid,fill opacity=0}, only marks]
table {%
2 38.6865625745935
};
\path [draw=black, fill=pink]
(axis cs:2.625,15.1483457229868)
--(axis cs:3.375,15.1483457229868)
--(axis cs:3.375,15.8535979370482)
--(axis cs:2.625,15.8535979370482)
--(axis cs:2.625,15.1483457229868)
--cycle;
\addplot [black]
table {%
3 15.1483457229868
3 14.9769260857937
};
\addplot [black]
table {%
3 15.8535979370482
3 15.8535979370482
};
\addplot [black]
table {%
2.8125 14.9769260857937
3.1875 14.9769260857937
};
\addplot [black]
table {%
2.8125 15.8535979370482
3.1875 15.8535979370482
};
\addplot [black, mark=o, mark size=1.5, mark options={solid,fill opacity=0}, only marks]
table {%
3 17.498206551896
};
\path [draw=black, fill=limegreen]
(axis cs:3.625,22.7446045604756)
--(axis cs:4.375,22.7446045604756)
--(axis cs:4.375,24.2070473943533)
--(axis cs:3.625,24.2070473943533)
--(axis cs:3.625,22.7446045604756)
--cycle;
\addplot [black]
table {%
4 22.7446045604756
4 21.271827294331
};
\addplot [black]
table {%
4 24.2070473943533
4 24.8233657305906
};
\addplot [black]
table {%
3.8125 21.271827294331
4.1875 21.271827294331
};
\addplot [black]
table {%
3.8125 24.8233657305906
4.1875 24.8233657305906
};
\path [draw=black, fill=forestgreen]
(axis cs:4.625,13.3637258791695)
--(axis cs:5.375,13.3637258791695)
--(axis cs:5.375,13.6830682365428)
--(axis cs:4.625,13.6830682365428)
--(axis cs:4.625,13.3637258791695)
--cycle;
\addplot [black]
table {%
5 13.3637258791695
5 13.1372104308748
};
\addplot [black]
table {%
5 13.6830682365428
5 13.6830682365428
};
\addplot [black]
table {%
4.8125 13.1372104308748
5.1875 13.1372104308748
};
\addplot [black]
table {%
4.8125 13.6830682365428
5.1875 13.6830682365428
};
\addplot [black, mark=o, mark size=1.5, mark options={solid,fill opacity=0}, only marks]
table {%
5 14.7598420359827
};
\path [draw=black, fill=darkgreen]
(axis cs:5.625,5.94491276389611)
--(axis cs:6.375,5.94491276389611)
--(axis cs:6.375,6.50974740109596)
--(axis cs:5.625,6.50974740109596)
--(axis cs:5.625,5.94491276389611)
--cycle;
\addplot [black]
table {%
6 5.94491276389611
6 5.73530645560373
};
\addplot [black]
table {%
6 6.50974740109596
6 6.73433909591233
};
\addplot [black]
table {%
5.8125 5.73530645560373
6.1875 5.73530645560373
};
\addplot [black]
table {%
5.8125 6.73433909591233
6.1875 6.73433909591233
};
\addplot [line width=1pt, black, dash pattern=on 9.25pt off 4pt]
table {%
0.625 2.58680682495297
1.375 2.58680682495297
};
\addplot [line width=1pt, black, dash pattern=on 9.25pt off 4pt]
table {%
1.625 27.3671122155182
2.375 27.3671122155182
};
\addplot [line width=1pt, black, dash pattern=on 9.25pt off 4pt]
table {%
2.625 15.8003974276729
3.375 15.8003974276729
};
\addplot [line width=1pt, black, dash pattern=on 9.25pt off 4pt]
table {%
3.625 23.0228674482705
4.375 23.0228674482705
};
\addplot [line width=1pt, black, dash pattern=on 9.25pt off 4pt]
table {%
4.625 13.5183965900627
5.375 13.5183965900627
};
\addplot [line width=1pt, black, dash pattern=on 9.25pt off 4pt]
table {%
5.625 6.00006064270732
6.375 6.00006064270732
};
\end{axis}

\end{tikzpicture}

